Joint Face Detection and Facial Motion Retargeting for Multiple Faces

Facial motion retargeting is an important problem in both computer graphics and vision, which involves capturing the performance of a human face and transferring it to another 3D character. Learning 3D morphable model (3DMM) parameters from 2D face images using convolutional neural networks is common in 2D face alignment, 3D face reconstruction etc. However, existing methods either require an additional face detection step before retargeting or use a cascade of separate networks to perform detection followed by retargeting in a sequence. In this paper, we present a single end-to-end network to jointly predict the bounding box locations and 3DMM parameters for multiple faces. First, we design a novel multitask learning framework that learns a disentangled representation of 3DMM parameters for a single face. Then, we leverage the trained single face model to generate ground truth 3DMM parameters for multiple faces to train another network that performs joint face detection and motion retargeting for images with multiple faces. Experimental results show that our joint detection and retargeting network has high face detection accuracy and is robust to extreme expressions and poses while being faster than state-of-the-art methods.

==> sec1_intro.tex <==
\vspace{-15pt}
\section{Introduction}
Facial gestures are an effective medium of non-verbal communication, and communication becomes more appealing through 3D animated characters. This has led to extensive research \cite{DDEregression,exprgen,hsieh2015unconstrained} in developing techniques to retarget human facial motion to 3D animated characters. The standard approach is to model human face by a 3D morphable model (3DMM)\cite{3DMM} and learn the weights of a linear combination of blendshapes that fits to the input face image. The learned ``expression" weights and ``head pose" angles are then directly mapped to semantically equivalent blendshapes of the target 3D character rig to drive the desired facial animation. Previous methods, such as \cite{DDEregression}, formulate 3DMM fitting as an optimization problem of regressing the 3DMM parameters from the input image. However, these methods require significant pre-processing or post-processing operations to get the final output.

Using deep convolution neural networks, recent works have shown remarkable accuracy in regressing 3DMM parameters from a 2D image. However, while 3DMM fitting with deep learning is frequently used in related domains like 2D face alignment\cite{3ddfa,adrian3Dfacealignment}, 3D face reconstruction\cite{CNN3DMMsynth,prn,dff,mobileface} etc., it hasn't been proven yet as an effective approach for facial motion retargeting. This is because 1) face alignment methods focus more on accurate facial landmark localization while face reconstruction methods focus more on accurate 3D shape and texture reconstruction to capture the fine geometric details. In contrast, facial retargeting to an arbitrary 3D character only requires accurate transfer of facial expression and head pose. However, due to the ambiguous nature of this ill-posed problem of extracting 3D face information from 2D image, both facial expression and head pose learned by those methods are generally \textit{sub-optimal} as they are not well decoupled from other information like identity. 2) Unlike alignment and reconstruction, retargeting often requires real-time tracking and transfer of the facial motion. However, existing methods for alignment and reconstruction are highly memory intensive and often involve complex rendering of the 3DMM as intermediate steps, thereby making these methods difficult to deploy on light-weight hardware like mobile phones. 

It is important to note that all previous deep learning based 3DMM fitting methods work on a single face image assuming face is already detected and cropped. To support multiple faces in a single image, a straightforward approach is to run a face detector on the image first to detect the all face regions and then perform the retargeting operations on each face individually. Such an approach, however, requires additional execution time for face detection and the computational complexity increases linearly with the number of faces in the input image. Additionally, tracking multiple faces with this approach becomes difficult when people move in and out from the frame or occlude each other. In the literature of joint face detection and alignment, existing methods \cite{JointDA_cascade, JointDA_cascade_mtl, Jointalignment} either use a random forest to predict the face bounding boxes and landmarks or adopt an iterative two-step approach to generate region proposals and predict the landmark locations in the proposed regions. However, these methods are primarily optimized for regressing accurate landmark locations rather than 3DMM parameters.

To this end, we divide our work into two parts. In the first part, we propose a multitask learning network to directly regress the 3DMM parameters from a well-cropped 2D image with a single face; we call this as Single Face Network (SFN). Our 3DMM parameters are grouped into: a) identity parameters that contain the face shape information, b) expression parameters that captures the facial expression, c) pose parameters that include the 3D rotation and 3D translation of the head and d) scale parameters that links the 3D face with the 2D image. We have observed that pose and scale parameters require global information while identity and expression parameters require different level of information, so we propose to emphasize on high level image features for pose and scale and the multi-scale features for identity and expression. Our network architecture is designed such that different layers embed image features at different resolutions, and these multi-scale features help in disentangling the parameter groups from each other. In the second part, we propose a single end-to-end trainable network to jointly detect the face bounding boxes and regress the 3DMM parameters for multiple faces in a single image. Inspired by YOLO\cite{yolo} and its variants\cite{yolov2,yolov3}, we design our Multiple Face Network (MFN) architecture that takes a 2D image as input and predicts the centroid position and dimensions of the bounding box as well as the 3DMM parameters for each face in the image. Unfortunately, existing publicly available multi-face image datasets provide ground truth for face bounding boxes only and not 3DMM parameters. Hence, we leverage our SFN to generate the weakly labelled ``ground truth" for 3DMM parameters for each face to train our MFN. Experimental results show that our MFN not only performs well for multi-face retargeting but also improves the accuracy of face detection. Our main contributions can be summarized as follows:
\begin{enumerate}
\itemsep0em 
\item We design a multitask learning network, specifically tailored for facial motion retargeting by casting the scale prior into a novel network topology to disentangle the representation learning. Such network has been proven to be crucial for both single face and multiple face 3DMM parameters estimation.
\item We present a novel top-down approach using an end-to-end trainable network to jointly learn the face bounding box locations and the 3DMM parameters from an image having multiple faces with different poses and expressions.
\item Our system is easy to deploy into practical applications without requiring separate face detection for pose and expression retargeting. Our joint network can be run in real-time on mobile devices without engineering level optimization, e.g. only 39ms on Google Pixel 2. 

\iffalse
\item We design a multitask learning framework that combines image features at different scales to disentangle and accurately predict different groups of 3DMM parameters.
\item We present a novel top-down approach to jointly learn the face bounding boxes and the 3DMM parameters from an image with multiple faces with different poses and expressions.
\item We present a weakly supervised method to generate ground truth 3DMM parameters for multiple faces to train our multi-face network.
\item We evaluate our networks on both image and video datasets and show that our method enables face tracking in videos with large inter-frame motion without the need for any additional face detection step.
\fi
\end{enumerate}


%To our best knowledge, no prior work has attempted to perform multiple 3DMM fitting for a single image with multiple faces using a single network.
%Inspired by the state-of-the-art object detection framework, such as Faster R-CNN  \cite{faster-rcnn}, YOLO\cite{yolo} and its variant\cite{yolov2,yolov3}, we propose an end-to-end learning system that can do joint face detection and 3DMM fitting tailored for face retargeting.
%Methods like Fast R-CNN \cite{fastrcnn} and YOLO \cite{yolo} have shown remarkable results in joint object detection and classification while achieving real time performance. 
%Similar methods have been applied to regress the 6D poses of multiple objects or humans in a single image \cite{Chen_2018_CVPR}, but to the best of our knowledge, no method has attempted to perform multiple 3DMM fitting to a single image using a single network.

==> sec2_relatedwork.tex <==
\vspace{-10pt}
\section{Related Work}

\subsection{2D Face Alignment and 3D Face Reconstruction}
Early methods like \cite{alignmentbytrees} used a cascade of decision trees or other regressors to directly regress the facial landmark locations from a face image. Recently, the approach of regressing 3DMM parameters using CNNs and fitting 3DMM to the 2D image has become popular. While Jourabloo et al. \cite{facealign3D2} use a cascade of CNNs to alternately regress the shape (identity and expression) and pose parameters, Zhu et al. \cite{3ddfa,pncc_new} perform multiple iterations of a single CNN to regress the shape and pose parameters together. These methods use large networks and require 3DMM in the network during testing, thereby requiring large memory and execution time. Regressing 3DMM parameters using CNNs is also popular in face reconstruction \cite{CNN3DMM,CNN3DMMsynth,cnnreconst,Tewari}. Richardson et al. \cite{Richardson} uses a coarse-to-fine approach to capture fine details in addition to face geometry. However, reconstruction methods also regress texture and focus more on capturing fine geometric details. For joint face alignment and reconstruction, \cite{prnet} regresses a position regression map from the image and \cite{nonlinear3dmm} regresses the parameters of a nonlinear 3DMM using an unsupervised encoder-decoder network. For joint face detection and alignment, recent methods either use a mixture of trees \cite{afwdatapaper} or a cascade of CNNs \cite{JointDA_cascade, JointDA_cascade_mtl}. In \cite{Jointalignment}, separate networks are trained to perform different tasks like proposing regions, classifying and regressing the bounding boxes from the regions, predicting the landmark locations in those regions etc. In \cite{hyperface}, region proposals are first generated with selective search algorithm and bounding box and landmark locations are regressed for each proposal using a multitask learning network. In contrast, we use a single end-to-end network to do join face detection and 3DMM fitting for face retargeting purposes.

\subsection{Performance-Based Animation}
Traditional performance capture systems (using either depth cameras or 3D scanners for direct mesh registration with depth data) \cite{AAM&depth,onlinemodeling,avataranimation_blendshapes} require complex hardware setup that is not readily available. Among the methods which use 2D images as input, the blendshape interpolation technique \cite{DDEregression,avataranimation_landmarks} is most popular. However, these methods require dense correspondence of facial points \cite{mocap} or user-specific adaptations \cite{realtime:animation:onthefly,Cao3d} to estimate the blendshape weights. Recent CNN based approaches either require depth input \cite{realtime:cnn:animation,SelfsupervisedCF} or regress character-specific parameters with several constraints \cite{exprgen}. Commercial software products like Faceshift \cite{faceshift}, Faceware \cite{faceware} etc. perform realtime retargeting but with poor expression accuracy \cite{exprgen}.

\subsection{Object Detection and Keypoint Localization}
In the literature of multiple object detection and classification, Fast RCNN \cite{rcnn} and YOLO \cite{yolo} are the two most popular methods with state-of-the-art performance. While \cite{rcnn} uses a region proposal network to get candidate regions before classification, \cite{yolo} performs joint object location regression and classification. Keypoint localization for multiple objects is popularly used for human pose estimation \cite{multiposenet,multipose} or object pose estimation \cite{object6d}. In case of faces, landmark localization for multiple faces can be done in two approaches: \textit{top-down approach} where landmark locations are detected after detecting face regions and \textit{bottom-up approach} where the facial landmarks are initially predicted individually and then grouped together into face regions. In our method, we adopt the top-down approach.

==> sec3_overview.tex <==
\section{Methodology}

\subsection{3D Morphable Model}

The 3D mesh of a human face can be represented by a multilinear 3D Morphable Model (3DMM) as
\begin{equation}
\mathcal{M} = \mathcal{V} \times \text{b}_{\text{id}} \times \text{b}_{\text{exp}}
\end{equation}
where $\mathcal{V}$ is the mean neutral face, $\text{b}_{\text{id}}$ are the identity bases and $\text{b}_{\text{exp}}$ are the expression bases. We use the face tensor provided by FacewareHouse \cite{facewarehouse} as 3DMM, where $\mathcal{V} \in \mathbb{R}^{11510 \times 3}$ denotes $11,510$ 3D co-ordinates of the mesh vertices, $\text{b}_{\text{id}}$ denotes 50 shape bases obtained by taking PCA over 150 identities and $\text{b}_{\text{exp}}$ denotes 47 bases corresponding to 47 blendshapes (1 neutral and 46 micro-expressions). To reduce the computational complexity, we manually mark 68 vertices in $\mathcal{V}$ as the facial landmark points based on \cite{afwdatapaper} and create a reduced face tensor $\hat{\mathcal{M}} \in \mathbb{R}^{204 \times 50 \times 47}$ for use in our networks. Given a set of identity parameters $w_\text{id} \in \mathbb{R}^{50 \times 1}$, expression parameters $w_\text{exp} \in \mathbb{R}^{47 \times 1}$, 3D rotation matrix $\mathbf{R} \in \mathbb{R}^{3 \times 3}$, 3D translation parameters $\mathbf{t} \in \mathbb{R}^{3 \times 1}$ and a scale parameter (focal length) $f$, we use weak perspective projection to get the 2D landmarks $\mathbf{P_{lm}} \in \mathbb{R}^{68\times2}$ as:
\begin{equation}
\mathbf{P_{lm}} = \begin{bmatrix}
    f       & 0 & 0 \\
    0      & f & 0
\end{bmatrix} [ \mathbf{R} * (\hat{\mathcal{M}}*w_\text{id}*w_\text{exp}) + \mathbf{t}]
\label{lm_eq}
\end{equation}
where $w_\text{exp}[1] = 1 - \sum_{i=2}^{47} w_\text{exp}[i]$ and $w_\text{exp}[i] \in [0,1], i = 2, \ldots, 47$. We use a unit quaternion $\mathbf{q} \in \mathbb{R}^{4 \times 1}$ \cite{pncc_new} to represent 3D rotation and convert it into rotation matrix for use in equation \ref{lm_eq}. Please note that, for retargeting purposes, we omit the learning of texture and lighting in the 3DMM.

\subsection{Multi-scale Representation Disentangling}
A straightforward way of holistically regressing all the 3DMM parameters together through a fully connected layer on top of one shared representation will not be optimal particularly for our problem where each group of parameters has strong semantic meanings. Intuitively speaking, head pose learning does not require detailed local face representations since it is fundamentally independent of skin texture and subtle facial expressions, which has also been observed in recent work on pose estimation \cite{tcdcn}. However, for identity learning, a combination of both local and global representations would be necessary to differentiate among different persons. For example, some persons have relatively small eyes but fat cheek while others have big eyes and thin cheek, so both the local features around the eyes and the overall face silhouette would be important to approximate the identity shape. Similarly, expression learning possibly requires even fine-grained granularity of different scales of representations. Single eye wink, mouth grin and big laugh clearly require three different levels of representations to differentiate them from other expressions.
%Recent method \cite{tcdcn} on pose estimation has shown satisfactory performance using just the eye, nose and mouth corner landmarks, which indicates that pose estimation requires global features. We also observe that the details from local features can confuse the pose estimation and end up causing the rotation to shake, while global features eliminate such noisy details, thus reduce the shaking. Identity or shape of the face depends on the face contour landmarks along with the corners, hence they require region-based features. However, estimation of expression parameters requires a dense arrangement of landmarks; therefore, requires local features from the input image. This motivated us to combine features at different scales for different parameters.
%The low level layers of a CNN learn the local features, whereas the high level layers capture the global information.

Another observation is, given the 2D landmarks of an image, there exist multiple combinations of 3DMM parameters that can minimize the 2D landmark loss. This ambiguity would cause additional challenges to the learning to favor the semantically more meaningful combinations. For examples, as shown in Fig. \ref{fig:decouple}, we can still minimize the 2D landmark loss by rotating the head and using different identity coefficients to accommodate the jaw left even without a strong jaw left expression coefficient. Motivated by both the multi-scale prior and the ambiguity nature of this problem, we designed a novel network structure that is specifically tailored for facial retargeting applications as illustrated in Fig. \ref{fig:teaser}, where pose is only learned through the final global features while expression learning depends on the concatenation of multi-layer representations.
\vspace{-10pt}
\paragraph{Disentangled Regularization} In addition to the above network design, we add a few regularization during the training to further enforce the disentangled representation learning. For example, for each face image, we can augment it by random translation/rotation perturbation to ask their resulting output to have the same identity and expression coefficients. Using image warping technique, we can re-edit the face image to slightly change the facial expression without hurting the pose and identity. Fig. \ref{fig:synthesis} shows a few such synthesized examples where their identity parameters need to be the same.

\begin{figure}[t]
\centering
\includegraphics[width=0.32\linewidth]{d1.jpg}
\includegraphics[width=0.32\linewidth]{d2.jpg}
\includegraphics[width=0.32\linewidth]{d3.jpg}
\caption{\textbf{left}: landmark projection from both meshes are exactly the same, \textbf{mid}: mesh with maximum jaw left, \textbf{right}: mesh without jaw left, but larger roll angle}
\label{fig:decouple}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.19\linewidth]{s0.jpg}
\includegraphics[width=0.19\linewidth]{s1.jpg}
\includegraphics[width=0.19\linewidth]{s2.jpg}
\includegraphics[width=0.19\linewidth]{s4.jpg}
\includegraphics[width=0.19\linewidth]{s6.jpg}
\caption{Synthesis image for regularization}
\label{fig:synthesis}
\end{figure}
%\addtolength{\textfloatsep}{-0.1in}
%We also observe that the combination of identity, expression and pose to generate landmark contains ambiguity. For example, it is possible to rotate the head and change identity to accommodate jaw left/right (Fig. \ref{fig:decouple}). It is also possible to close eye with identity blendshape (Fig. \ref{decouple2}). The identity should have nothing to do with expression, and always predict the neutral expression first before combining with expression parameters. Hence disentangling of the parameters is necessary to prevent the network from learning meaningless combinations and can be achieved by training 3 different networks for each task. However, we chose to share some of the layers to reduce computation cost, and easily integrate with the multi-scale prior.

==> sec4_methodology.tex <==
%\section{Methodology}
\subsection{Single Face Retargeting Network}\label{sec:sfn}
When the face bounding box is given, we can train a single face retargeting network to output 3DMM parameters for each cropped face image using the above proposed network structure. Fortunately, many public datasets \cite{300w, facewarehouse, LFWTech, 3ddfa} already provide bounding boxes along with 68 2D facial landmark points. To encourage disentangling, we fit 3DMM parameters for each cropped single face image using the optimization method of \cite{adrian3Dfacealignment} and treat them as ground truth for our network in addition to the landmarks. Although individual optimization may result in over-fitting and noisy ground truth, our network can intrinsically focus more on the global common patterns from the training data. To achieve this, we initially train with a large weight on the L1 loss with respect to the ground truth ($g$), and then gradually decay this weight to trust more on the 2D landmarks loss, as shown in the following loss function:
%The common approach for solving face retargeting is to have a dedicated network for face detection, and another network to retarget each of the face patch. Many public datasets \cite{300w, facewarehouse, LFWTech, 3ddfa} provide bounding box or already crop the face patch along with 68 facial landmark points. Given these landmarks, we can optimize 3DMM coefficients \cite{adrian3Dfacealignment} and incorporate them as ground truth into our loss function by mean absolute error. We found that these optimized coefficients are important during the early epochs of training to quickly guide the learner towards 3D representation. However, the limitation of \cite{adrian3Dfacealignment} lies in a single image input. Optimizing on single image can easily lead to local optima. Optimizing on multiple images is possible in theory, however, it is computational expensive and usually require a good prior (such as all these images are the same person). Deep networks, on the other hand, can be trained on large training sets which increases the tolerance for local noise from individual images. We choose to steadily learn the 2D landmarks by root mean square error while decaying the 3DMM coefficients loss. The combined loss function is:
\begin{multline}
\tau * \Bigg\{\frac{1}{50}\sum_{i = 1}^{50}|w_{\text{id}_i} - {w}^g_{\text{id}_i}|
+\frac{1}{46}\sum_{i = 1}^{46}|w_{\text{exp}_i} - {w}^g_{\text{exp}_i}|    \\
+\frac{1}{4}\sum_{i = 1}^{4}|\mathbf{R}_i - \mathbf{R}^g_i|\Bigg\}
+ \sqrt{\frac{1}{68}\sum_{i = 1}^{68}(\mathbf{P}_{\text{lm}_i} - \mathbf{P}^g_{\text{lm}_i})^2}
\label{eq:sfn_loss}
\end{multline}
where $\tau$ denotes decay parameter with respect to epoch. We choose $\tau$ = 10/epoch across all experiments. Note that, although we drop the 3D translation and scale ground truth loss to allow 2D translation and scaling augmentation, the translation and scale parameters can still be learned by the 2D landmark loss.

\iffalse
The network has two stages. The first stage takes a 2D human face image of size $128 \times 128$ pixels as input and predicts the identity, expression, pose and scale parameters of the 3DMM as output. The optional second stage is a light-weight extension that takes the eye and mouth regions of the image as input and refines the expression parameters predicted by the first stage.

\baoyuan{I think we should move this single-scale network to the implementation details, only discuss the multi-scale network}
\fi

\iffalse
\begin{figure}[]
\centering
\includegraphics[width=1.0\linewidth]{images/single_scale_model.jpg}
\caption{Single scale face retargeting network. The final feature map is connected to fully connected layer to respect the dimension of each 3DMM parameters.}
\label{fig:sfn}
\end{figure}
\fi
\subsection{Joint Face Detection and Retargeting}
Our goal is to save computation cost by performing both face detection and 3DMM parameter estimation simultaneously instead of sequentially running a separate face detector and then single face retargeting network on each face separately. The network could potentially also benefit from the cross domain knowledge, especially for detection task, where introducing 3DMM gives the prior on how the face should look like in 3D space which complements the 2D features in separate face detection framework.

Inspired by YOLO \cite{yolo}, our joint network is designed to predict 3DMM parameters for each anchor point in additional to bounding box displacement and objectness. We divide the input image into $9 \times 9$ grid and predict a vector of length $4 + 1 + (50 + 46 + 4 + 3 + 1) =  109$ for a bounding box in each grid cell. Here 4 denotes 2D co-ordinates of the centroid, width and height of the face bounding box, 1 denotes the confidence score for the presence of a face in that cell and the rest denote the 3DMM parameters for the face in the cell. We also adopt the method of starting with 5 anchor boxes as bounding box priors. Our final loss function is the summation of equation \ref{eq:sfn_loss} across all grids and anchors, as shown in the following:
%Although most training sets provide face bounding box, it is not trivial to train a face detector to handle all kind of identity, expression and especially large pose. Another approach could be detecting only the first frame bounding box(es) and use the past frame bounding box(es) to generate current frame 3DMM coefficients to obtain landmarks and ultimately track the bounding box(es). This tracking approach, however, quickly becomes complicated when people move in and out from the frame or occlude each other. A face detector in the background thread is still usually required to ensure reliability. Moreover, we need to run tracking network per face which linearly increase the computation time. As the practical application requires face detector one way or another, we propose to jointly train face detector with retargeting. The goal is to save computation cost by predicting both tasks at the time. The network could potentially also benefits from the cross domain knowledge, especially in detection task. Detector always learn from 2D bounding box which may not be enough for large pose. Introducing 3DMM gives the prior on how the face should look like in 3D space, and implicitly provide 3D bounding box through the dense mesh as well.
%We choose to naturally integrate retargeting into YOLO \cite{yolo} by predicting 3DMM parameters for each anchor. We divide the input image into $9 \times 9$ grid and predict a vector of length $4 + 1 + (50 + 46 + 4 + 3 + 1) =  109$ for a bounding box in each grid cell. Here, 4 denotes the 2D co-ordinates of the centroid, width and height of the face bounding box, 1 denotes the confidence score for the presence of a face in that cell and the rest are the 3DMM parameters for the face in the cell. We also adopt the method of starting with 5 anchor boxes as bounding box priors. The $x,y$ co-ordinates of the centroid and the width and height of a bounding box are calculated in the same manner as in \cite{yolo} and we use the same loss functions for these values. We obtain the 3DMM ground truth by running our single face retargeting network. The revised lose function is the summation of \ref{eq:sfn_loss} across all grids and anchors.
\iffalse
\begin{equation*}
    b_{\text{id}} = t_{v_{1-50}}; \; b_{\text{exp}} = \sigma (t_{v_{51-97}})
\end{equation*}
\begin{equation*}
    b_{\textbf{R}} = t_{v_{98-101}}; \; b_{\textbf{t}} = t_{v_{102-104}}; \; b_{\text{f}} = \sigma (t_{v_{105}})
\end{equation*}
\begin{equation*}
    b_{\text{lm}_x} = b_x + b_w * b_{\Hat{\text{lm}}_x}; \; b_{\text{lm}_y} = b_y + b_h * b_{\Hat{\text{lm}}_y}
\end{equation*}
where $\sigma$ denotes sigmoid function and $b_{\Hat{\text{lm}}}$ are the initial landmarks obtained using equation \ref{lm_eq}. The loss function for the 3DMM parameters is:
\fi
% \biggl( 
% \biggr)
\begin{multline}
\tau * \Bigg\{\frac{1}{50}\sum_{j = 1}^{9^2} \sum_{k = 1}^{5}\sum_{i = 1}^{50}\mathbbm{1}_{ijk}|w_{\text{id}_{ijk}} - {w}^g_{\text{id}_{ijk}}|    \\
+\frac{1}{46}\sum_{j = 1}^{9^2} \sum_{k = 1}^{5}\sum_{i = 1}^{46}\mathbbm{1}_{ijk}|w_{\text{exp}_{ijk}} - {w}^g_{\text{exp}_{ijk}}|    \\
+\frac{1}{4}\sum_{j = 1}^{9^2} \sum_{k = 1}^{5}\sum_{i = 1}^{4}\mathbbm{1}_{ijk}|\mathbf{R}_{ijk} - \mathbf{R}^g_{ijk}|\Bigg\} \\ 
+ \sqrt{\frac{1}{68}\sum_{j = 1}^{9^2} \sum_{k = 1}^{5}\sum_{i = 1}^{68}\mathbbm{1}_{ijk}(\mathbf{P}_{\text{lm}_{ijk}} - \mathbf{P}^g_{\text{lm}_{ijk}})^2}\
\end{multline}
\label{eq:yolo_loss}
where $\mathbbm{1}_{ijk}$ denotes whether a $k$th bounding box predictor in cell $j$ contains a face. Since there are no publicly available multi-face datasets that provide both bounding box location and 3DMM parameters for each face, for proof-of-concept, we obtain the 3DMM ground truth by running our single face retargeting network on each face separately. The $x,y$ co-ordinates of the centroid and the width and height of a bounding box are calculated in the same manner as in \cite{yolo} and we use the same loss functions for these values.









% \subsection{Loss function}

% The loss function to be optimized then becomes:
% \begin{equation}
% \mathcal{L}_{\text{P}_{2D}} = ||\textbf{P}_{\text{2D}}^\text{gt} - \mathbf{P}_{\text{2D}}^\text{pred}||_2
% \label{eq:2D}
% \end{equation}
% where for each of the $L$ facial landmarks, \textbf{Pr} is the camera projection matrix that projects the $k$-th vertex $v_k$ of the rotated and translated 3D mesh onto the 2D plane and match it with the corresponding ground truth 2D landmark $p_k^{2d}$. 
% \begin{equation}
% \sum_{k=1}^{L} ||[R(Bw^T)+t]^{v_k} - p_k^{3d}||_2^2
% \label{eq:3D}
% \end{equation}
% which is a modified version of equation \ref{eq:2D}.
% We use the FacewareHouse model of 11K vertices $\times$ 46 blendshapes $\times$ 150 identities, hence the weight vector to compute the user-specific blendshapes is a 150-dimensional vector, say $x$. Also, the camera projection matrix has only one unknown - the focal length $f$. Hence, the output of our neural network model will now be a 202-dimensional vector - 50 for identity, 46 for blendshapes, 3 for rotation, 2 for translation and 1 for scale (focal length). We would like to point out that the identity weight vector and the scale factor is only needed for the joint optimization during training and will not be required for retargeting during testing.\\
% The advantage of this approach over the previous one is that the results don't depend on the accuracy of the underlying method used to generate the ground truth data. We just need a database of face images with corresponding labeled facial landmarks.

%  We use an existing approach, more specifically \cite{DDEregression}, to predict the parameters and use them as ground truth to train our deep network. This allows us to leverage the large number of publicly available face databases, since the only input needed is face images. The loss function to be optimized can simply be the L2 loss between the predicted and ground truth parameters, and we can have additional loss terms for temporal coherence etc. We tried weighting the L1 expression coefficient loss by the importance of each blendshape (more the displacement with respect to neutral, more is the weight) and also tried KL divergence loss with L1-normalized coefficients, but finally simple L1 loss works best. The total loss is given by
% \begin{equation}
% \begin{split}
% \lambda_\text{id} \mathcal{L_\text{id}} + \lambda_\text{exp}^1 \mathcal{L_\text{exp}}^1 + 
% \lambda_\text{exp}^2 \mathcal{L_\text{exp}}^2 + \lambda_\text{R} \mathcal{L_\text{R}} + \lambda_{\text{P}_{2D}} \mathcal{L}_{\text{P}_{2D}} \\ + \lambda_{\text{P}_{3D}}^\text{eye} \mathcal{L}_{\text{P}_{3D}}^\text{eye} +
% \lambda_{\text{P}_{3D}}^\text{mouth} \mathcal{L}_{\text{P}_{3D}}^\text{mouth}
% \end{split}
% \end{equation}
% The loss weights are decided based on their importance. We use $\lambda_\text{id}$ = 2, $\lambda_\text{exp}^1$ = 5, $\lambda_\text{exp}^2$ = 10, $\lambda_\text{R}$ = 3, $\lambda_{\text{P}_{2D}}$ = 1, $\lambda_{\text{P}_{3D}}^\text{eye}$ = $\lambda_{\text{P}_{3D}}^\text{mouth}$ = 100.

==> sec5_implementation.tex <==
\section{Experimental Setup}

\subsection{Datasets}
\iffalse
The authors of \cite{DDEregression} provide the corresponding 68 landmarks for both the datasets.
Front camera images captured by mobile phones have lower resolution and image quality and are strikingly different from rear camera images because of perspective distortion due to proximity of the face to the camera. As a result, networks trained on in-the-wild face images do not perform well with the front camera. To overcome this issue, we captured the facial performance of several users using front camera and annotated each frame of the captured videos with 68 landmarks using the method proposed in \cite{adrian3Dfacealignment}.\fi

For single face retargeting, we combine multiple datasets to have a good training set for accurate prediction of each group of 3DMM parameters. 300W-LP contains many large poses and Facewarehouse is a rich dataset for expressions. The ground truth 68 2D landmarks provided by these datasets are used to obtain 3DMM ground truth by \cite{adrian3Dfacealignment}. LFW and AFLW2000-3D are used as test sets for static images and 300VW is used as test set for tracking on videos. For multiple face retargeting, AFW has ground truth bounding boxes, pose angles and 6 landmarks and is used as a test set for static images, while FDDB and WIDER only provide bounding box ground truth and are therefore used for training (WIDER test set is kept separate for testing). Music videos dataset is used to test our MFN performance on videos. We remove all images with more than 20 faces and also remove faces whose bounding box dimensions are \textless2\% of the image dimensions from both the training and test sets. This mainly includes faces in the background crowd with size less than 5$\times$5 pixels. The reason is that determining the facial expressions for such small faces is ambiguous even for human eyes and hence retargeting is not meaningful.
More dataset details are summarized in Table \ref{tab:dataset}. We use an 80-20 split of the training set for training and validation. To measure the performance of expression accuracy, we manually collect an expression test set by selecting those extreme expression images (Fig. \ref{fig:result4}). The number of images in each of the expression categories are: eye close: 185, eye wide: 70, brow raise: 124, brow anger: 100, mouth open: 81, jaw left/right: 136, lip roll: 64, smile: 105, kiss: 143, total: 1008 images.


\begin{table}[t]
\begin{tabular}{|l|l|c|c|}
\hline
\multicolumn{2}{|c|}{\textbf{Dataset}} & \multicolumn{1}{c|}{\textbf{\#images}} & \multicolumn{1}{c|}{\textbf{\#faces}} \\ \hline
\multirow{5}{*}{SFN}      & 300W-LP \cite{300w,3ddfa} & 61225 & 61225 \\ \cline{2-4} 
                          & FacewareHouse \cite{facewarehouse} & 5000  & 500 \\ \cline{2-4} 
                          & LFW \cite{LFWTech} & 12639  & 12639  \\ \cline{2-4} 
                          & AFLW2000-3D \cite{3ddfa} & 2000  & 2000 \\ \cline{2-4} 
                          & 300VW \cite{300VW} & 114 (videos)  & 218K\\
                          \hline
                          
\multirow{4}{*}{MFN}      & FDDB \cite{fddb} & 2845 & 5171 \\ \cline{2-4} 
                          & WIDER \cite{wider} & 11905 & 56525 \\ \cline{2-4} 
                          & AFW \cite{afwdatapaper} & 205 & 1000 \\ \cline{2-4} 
                          & Music videos \cite{musicvideo} & 8 (videos) & - \\
                          \hline
\end{tabular}
\caption {Number of images or videos and faces for each dataset used in training and testing of our networks.}
\label{tab:dataset}
\end{table}
%\addtolength{\textfloatsep}{-0.4in}



\iffalse
\subsection{Face Tracking for SFN}
For a video, we initially feed the entire image into the network and keep shrinking the bounding box over time until it fits the face. Then we set the bounding box of the current frame using the boundaries of the 2D landmarks of the previous frame and perform retargeting on a frame-by-frame basis. Hence, unlike other methods, our method does not require a separate face detection module at any instant. Finally, we smooth the predicted parameters using a Kalman filter.
\fi

%\vspace{-6mm}

\subsection{Evaluation Metrics}
We use 4 metrics: 1) average precision (AP) with different intersection-over-union thresholds as defined in \cite{yolov3} to evaluate our MFN performance for face detection, 2) normalized mean error (NME) defined as the Euclidean distance between the predicted and ground truth 2D landmarks averaged over 68 landmarks and normalized by the bounding box dimensions, 3) area under the curve (AUC) of the Cumulative Error Distribution curve for landmark error normalized by the diagonal distance of ground truth bounding box \cite{Jointalignment}, and 4) expression metric defined as the mean absolute distance between the predicted expression parameters with respect to the ground truth, which is 1 in our case following the practice of \cite{facewarehouse}. 
%We propose explicit expression evaluation because several expressions such as eye close, eye wide etc. do not significantly move the landmarks, and thus the landmark error will be too small to justify.

\iffalse
\begin{table}[h]
\begin{tabular}{l|l|l|l|l|l|}
\cline{2-6}
   & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Eye\\ Close\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Eye\\ Wide\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Brow\\ Raise\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Brow\\ Anger\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Mouth\\ Wide\end{tabular}}} \\ \hline
\multicolumn{1}{|l|}{\textbf{\#images}} & 100     & 100     & 100     & 100     & 100     \\ \hline
\end{tabular}
\end{table}

\begin{table}[h]
\begin{tabular}{l|l|l|l|l|l|}
\cline{2-6}
   & \multicolumn{1}{c|}{\textbf{Jaw}} & \multicolumn{1}{c|}{\textbf{LipRoll}} & \multicolumn{1}{c|}{\textbf{Smile}} & \multicolumn{1}{c|}{\textbf{Kiss}} & \multicolumn{1}{c|}{\textbf{Total}} \\ \hline
\multicolumn{1}{|l|}{\textbf{\#images}} & 100  & 100   & 100   & 100  & 100   \\ \hline
\end{tabular}
\end{table}
\fi


\subsection{Implementation Details}

\subsubsection{Training Configuration}
 Our networks are implemented in Keras \cite{chollet2015keras} with Tensorflow backend and trained using Adam optimizer with batch size 32. The initial learning rate ($10^{-3}$ for SFN and $10^{-4}$ for MFN) is decreased by 10 times (up to $10^{-6}$) when the validation loss does not change over 5 consecutive epochs. Training takes about a day on a Nvidia GTX 1080 for each network. For data augmentation, we use random scaling in the range [0.8,1.2], random translation of 0-10\%, color jitter and in-plane rotation. These augmentation techniques improve the performance of SFN and also help in generating more accurate ground truth for individual faces for MFN.

\subsubsection{Single Face Retargeting Architecture}
%Our network jointly predicts identity, expression and pose parameters.
Our network takes 128x128 resized image as input. In the first layer, we use a $7 \times 7$ convolution layer with 64 filters and stride 2 followed by a $2\times2$ maxpooling layer to capture the fine details in the image. The following layers are made up of Fire Modules(FM) of SqueezeNet \cite{SqueezeNet} (with 16 and 64 filters in squeeze and expand layers respectively) and squeeze-and-excite modules(SE) of \cite{SEnet} in order to compress the model size and reduce the model execution time without compromising the accuracy. At the end of network, we use a global average pooling layer followed by fully connected (FC) layers to generate the parameters. The penultimate FC layers each has 64 units with ReLU activation and sigmoid activation is used at the end of the last expression branch's FC layer  to restrict the values between 0 and 1. To realize the multiscale prior and the disentangled learning, we concatenate the features at different scales and form separate branches for each group of parameters. The extra branches are built with the same blocks as the main branch, but we reduce the channel size by half to restrict the extra computation cost.

\subsubsection{Joint Detection and Retargeting Architecture}
Our joint detection and retargeting network architecture is similar to Tiny DarkNet \cite{yolo} with the final layer changed to predict a tensor of size $9\times 9 \times 5 \times 109$. However, since we only have one object class (face) in our problem, we reduce the number of filters in each layer to a quarter of their original values. For multi-scale version, we change the input image size to $288 \times 288$ and extend the multi-scale backbone for single face retargeting by changing the output of each branch to accommodate grid output (Fig. \ref{fig:teaser}). The pose branch outputs change from 4 ($R$) + 3 ($T$) + 1 ($f$) = 8 to $9\times 9 \times 5 \times 8$. The expression branch outputs change from 46 to $9\times 9 \times 5 \times 46$, and identity branch outputs change from 50 to $9\times 9 \times 5 \times 50$. One extra branch is also added to output objectness and bounding box location ($9\times 9 \times 5 \times (4+1)$). In total, multi-scale version outputs the same dimension as single-scale, but the output channels are split with respect to each type of branch.

==> sec6_results.tex <==

\iffalse
\begin{table*}[h]
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{Model}}} & \multicolumn{4}{c|}{\textbf{Evaluation}}        & \multicolumn{4}{c|}{\textbf{Resource}}        \\ \cline{2-9} 
\multicolumn{1}{|c|}{}  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Single Face\\ NME (\%)\end{tabular}} & \multicolumn{3}{c|}{Multi Face}    & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Size\\ (MB)\end{tabular}} & \multicolumn{3}{c|}{Speed (second)}    \\ \cline{3-5} \cline{7-9} 
\multicolumn{1}{|c|}{}  &      & \multicolumn{1}{l|}{AP} & \multicolumn{1}{l|}{AP50} & \multicolumn{1}{l|}{AP75} &     & \multicolumn{1}{l|}{1 face} & \multicolumn{1}{l|}{5 faces} & \multicolumn{1}{l|}{10 faces} \\ \hline
(1) YOLO   & -     & 40.0  &  &  & 20.0     & 1.0  & 1.0  & 1.0  \\ \hline
(2) SFN   & 2.21     & \multicolumn{3}{c|}{-}    & 5.0     & 1.1  & 1.5  & 2.0  \\ \hline
(3) SFN + Pose  & 1.91     & \multicolumn{3}{c|}{-}    & 5.0     & 1.1  & 1.5  & 2.0  \\ \hline
(4) SFN + ID  & 1.91     & \multicolumn{3}{c|}{-}    & 5.0     & 1.1  & 1.5  & 2.0  \\ \hline
(5) SFN + Exp  & 1.91     & \multicolumn{3}{c|}{-}    & 5.0     & 1.1  & 1.5  & 2.0  \\ \hline
(6) SFN + ID + EXP  & 1.91     & \multicolumn{3}{c|}{-}    & 5.0     & 1.1  & 1.5  & 2.0  \\ \hline
(7) SFN + ID + Pose  & 1.91     & \multicolumn{3}{c|}{-}    & 5.0     & 1.1  & 1.5  & 2.0  \\ \hline
(8) SFN + Exp + Pose  & 1.91     & \multicolumn{3}{c|}{-}    & 5.0     & 1.1  & 1.5  & 2.0  \\ \hline
(9) SFN + ID + EXP + Pose  & 1.91     & \multicolumn{3}{c|}{-}    & 5.0     & 1.1  & 1.5  & 2.0  \\ \hline
(10) YOLO + GT from (2)  & 4.0     & 35.0  &  &  & 20.0     & 1.0  & 1.0  & 1.0  \\ \hline
(11) YOLO + GT from (9)  & 2.5     & 45.0  &  &  & 20.0     & 1.0  & 1.0  & 1.0  \\ \hline
(12) Compressed YOLO + GT from (9)  & 3.0     & 40.0  &  &  & 5.0     & 0.1  & 0.1  & 0.1  \\ \hline
\end{tabular}
\caption{something}
\end{table*}
\fi

\begin{figure}[t]
\centering
\begin{subfigure}[t]{1.0\linewidth}
\centering
\begin{subfigure}[t]{0.19\textwidth}
\centering
%\footnotesize input-1\\
\includegraphics[width = 0.95\textwidth, height = 0.065\textheight]{images/layer1.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.19\textwidth}
\centering
%\footnotesize input-3\\
\includegraphics[width = 0.95\textwidth, height = 0.065\textheight]{images/ss1.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.19\textwidth}
\centering
%\footnotesize input-2\\
\includegraphics[width = 1.0\textwidth, height = 0.065\textheight]{images/exp1.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.19\textwidth}
\centering
%\footnotesize input-3\\
\includegraphics[width = 1.0\textwidth, height = 0.065\textheight]{images/id1.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.19\textwidth}
\centering
%\footnotesize input-3\\
\includegraphics[width = 1.0\textwidth, height = 0.065\textheight]{images/pose1.jpg}
\end{subfigure}
%\caption{Output of 1st stage of SFN}
\end{subfigure}
\begin{subfigure}[t]{1.0\linewidth}
\centering
\begin{subfigure}[t]{0.19\textwidth}
\centering
%\footnotesize input-1\\
\includegraphics[width = 0.95\textwidth, height = 0.065\textheight]{images/layer2.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.19\textwidth}
\centering
%\footnotesize input-3\\
\includegraphics[width = 0.95\textwidth, height = 0.065\textheight]{images/ss2.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.19\textwidth}
\centering
%\footnotesize input-2\\
\includegraphics[width = 1.0\textwidth, height = 0.065\textheight]{images/exp2.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.19\textwidth}
\centering
%\footnotesize input-3\\
\includegraphics[width = 1.0\textwidth, height = 0.065\textheight]{images/id2.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.19\textwidth}
\centering
%\footnotesize input-3\\
\includegraphics[width = 1.0\textwidth, height = 0.065\textheight]{images/pose2.jpg}
\end{subfigure}
%\caption{Output of 1st stage of SFN}
\end{subfigure}
\caption{Visualization of learned features. From left to right in each row: input image, features for single scale SFN, features for expression branch of multi-scale SFN, features for identity branch of multi-scale SFN, features for pose branch of multi-scale SFN.}
\label{fig:layeroutputs}
\end{figure}

\section{Results}
\subsection{Importance of Multi-Scale Representation} %Disentangling}
Our multi-scale network design reduces the load on the network to learn complex features by allowing the network to concentrate on different image features to learn different parameters unlike the single scale design. In Fig. \ref{fig:layeroutputs}, we see that single scale network learns generic facial features that combines the representations for identity, expression and pose. On the other hand, multi-scale network learns different levels of representation (pixel-level detailed features for expression, region level features for identity and global aggregate features for pose). We have randomly chosen only 25 filter outputs at level 3 of our SFN for clearer visualization. Table \ref{table:full} shows that our multi-scale design not only reduces NME for single face images using SFN but also improves the performance of MFN in terms of both NME (by generating a better weakly supervised ground truth) and AP for detection. Clearly, different feature representations are crucial to accurately learn different groups of parameters. By reducing the network load, this design also allows model compression so that multi-scale networks can be of comparable size with respect to single scale networks while having better accuracy. Fig. \ref{fig:howfarcomparison} shows that the multi-scale design predicts more accurate expression parameters (first row has correct landmarks for closed eyes) and identity parameters (second row has correct landmarks that fit the face shape) while being robust to large poses (second row), illumination (first row) and occlusion (third row).

\begin{table}[t]
\small
\begin{tabular}{|l|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{Model}} & \multicolumn{4}{c|}{Evaluation} \\ 
\cline{2-5} \multicolumn{1}{|c|}{}  &  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}NME\\ (\%)\end{tabular}} & \multicolumn{3}{c|}{Multi Face}  \\ 
\cline{3-5} \multicolumn{1}{|c|}{}  &      & \multicolumn{1}{l|}{AP} & \multicolumn{1}{l|}{AP50} & \multicolumn{1}{l|}{AP75} \\ \hline
(1) MFN (detection only)  & - & 92.1 & 99.2 & 94.3\\ \hline
(2) Single scale SFN & 2.16 & - & - & -\\ \hline
%(3) SFN + Pose  & 3.0 & 40.0 & - & - \\ \hline
%(4) SFN + ID  & 3.0 & 40.0 & - & - \\ \hline
%(5) SFN + Exp  & 3.0 & 40.0 & - & - \\ \hline
%(6) SFN + ID + EXP  & 3.0 & 40.0 & - & - \\ \hline
%(7) SFN + ID + Pose  & 3.0 & 40.0 & - & -  \\ \hline
%(8) SFN + Exp + Pose  & 3.0 & 40.0 & - & - \\ \hline
(3) Multi-scale SFN  & 1.91 & - & - & - \\ \hline
(4) SS-MFN + GT from (2) & 2.89 & 97.5 & 99.8 & 98.1  \\ \hline
(5) SS-MFN + GT from (3)  & 2.65 & 98.2 & 100 & 98.9  \\ \hline
(6) MS-MFN + GT from (3)  & 2.23 & 98.8 & 100 & 99.3\\ \hline
\end{tabular}
\caption{Quantitative evaluation of our SFN and MFN. SS-MFN and MS-MFN denote single scale and multi-scale MFN respectively. NME values are calculated for LFW (single faces) and AP values are calculated for AFW.}
\label{table:full}
\end{table}

\begin{figure}[t]
\centering
\begin{subfigure}[t]{1.0\linewidth}
\centering
\begin{subfigure}[t]{0.24\textwidth}
\centering
%\footnotesize input-1\\
\includegraphics[width = 1.0\textwidth, height = 0.08\textheight]{images/res3.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
\centering
%\footnotesize input-2\\
\includegraphics[width = 1.0\textwidth, height = 0.08\textheight]{images/res31.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
\centering
%\footnotesize input-3\\
\includegraphics[width = 1.0\textwidth, height = 0.08\textheight]{images/stage1res3.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
\centering
%\footnotesize input-3\\
\includegraphics[width = 1.0\textwidth, height = 0.08\textheight]{images/stage2res3.jpg}
\end{subfigure}
%\caption{Input images with ground truth landmarks}
\end{subfigure}

\begin{subfigure}[t]{1.0\linewidth}
\centering
\begin{subfigure}[t]{0.24\textwidth}
\centering
%\footnotesize input-1\\
\includegraphics[width = 1.0\textwidth, height = 0.08\textheight]{images/res5.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
\centering
%\footnotesize input-2\\
\includegraphics[width = 1.0\textwidth, height = 0.08\textheight]{images/res51.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
\centering
%\footnotesize input-3\\
\includegraphics[width = 1.0\textwidth, height = 0.08\textheight]{images/stage1res5.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
\centering
%\footnotesize input-3\\
\includegraphics[width = 1.0\textwidth, height = 0.08\textheight]{images/stage2res5.jpg}
\end{subfigure}
%\caption{Output of 1st stage of SFN}
\end{subfigure}

\begin{subfigure}[t]{1.0\linewidth}
\centering
\begin{subfigure}[t]{0.24\textwidth}
\centering
%\footnotesize input-1\\
\includegraphics[width = 1.0\textwidth, height = 0.08\textheight]{images/res6.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
\centering
%\footnotesize input-2\\
\includegraphics[width = 1.0\textwidth, height = 0.08\textheight]{images/res61.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
\centering
%\footnotesize input-3\\
\includegraphics[width = 1.0\textwidth, height = 0.08\textheight]{images/stage2res6.jpg}e
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
\centering
%\footnotesize input-3\\
\includegraphics[width = 1.0\textwidth, height = 0.08\textheight]{images/stage2res6.jpg}
\end{subfigure}
%\caption{Output of 2nd stage of SFN}
\end{subfigure}
\caption{2D Face Alignment results for AFLW2000-3D. First column: original image with ground truth landmarks; Second column: results using \cite{adrian3Dfacealignment}; Third column: our single scale SFN; Last column: our multi-scale SFN.}
\label{fig:howfarcomparison}
\end{figure}

\subsection{Comparison with 2D Alignment Methods}
Even though we aim to predict the 3DMM parameters for retargeting applications, our model can naturally serve the purpose for 2D face alignment (via 3D). Therefore, we can evaluate our model from the performance of 2D alignment perspective. Table \ref{table:aflw_nme} compares the performance of our single scale and multi-scale SFN with state-of-the-art 2D face alignment methods (compared under the same settings). As can be seen, our model achieves much smaller errors compared to most of the methods that are dedicated for precise landmark localization. While PRN \cite{prn} has lower NME, its network size is 80 times bigger than ours and takes 9.8ms on GPU compared to $<$1ms required by our network. In addition to evaluations on static images, we also measure the face tracking performance in a video using our SFN. We set the bounding box of the current frame using the boundaries of the 2D landmarks detected in the previous frame and perform retargeting on a frame-by-frame basis. Table \ref{table:300vw_auc} compares the AUC values on 300VW dataset for three scenarios categorized by the dataset (compared under the same settings). Our method performs significantly better than other methods (about 9\% improvement over the second best method for Scenario 3) with negligible failure rate because extensive data augmentation helps our tracking algorithm to quickly recover from failures.

\begin{table}[t]
\small
    \centering
    \begin{tabular}{|c||c|c|c|c|}
    \hline
     Method  &  [0\degree,30\degree] & [30\degree,60\degree] & [60\degree,90\degree] & Mean\\
     \hline
     SDM \cite{sdm}  &  3.67 & 4.94 & 9.67 & 6.12 \\
     \hline
     3DDFA \cite{3ddfa} & 3.78 & 4.54 & 7.93 & 5.42\\
     \hline
     3DDFA2 \cite{3ddfa} & 3.43 & 4.24 & 7.17 & 4.94\\
     \hline
     Yu et al. \cite{Yu2017LearningDF} & 3.62 & 6.06 & 9.56 & 6.41\\
     \hline
     3DSTN \cite{FasterTR} & 3.15 & 4.33 & 5.98 & 4.49\\
     \hline
     DFF \cite{dff}  & 3.20 & 4.68 & 6.28 & 4.72 \\
     \hline
     PRN \cite{prn} & 2.75 & 3.51 & 4.61 & 3.62\\
     \hline
     SS-SFN (ours) & \textbf{3.09} & \textbf{4.27} & \textbf{5.59} & \textbf{4.31}\\
     \hline
     MS-SFN (ours) & \textbf{2.91} & \textbf{3.83} & \textbf{4.94} & \textbf{3.89}\\
     \hline
    \end{tabular}
    \caption{Comparison of NME(\%) for 68 landmarks for AFLW2000-3D (divided into 3 groups based on yaw angles). 3DDFA2 refers to 3DDFA+SDM \cite{3ddfa}.}
    \label{table:aflw_nme}
\end{table}

\begin{table}[t]
\small
    \centering
    \begin{tabular}{|c||c|c|c|}
    \hline
     Method & Scenario 1 & Scenario 2 & Scenario 3\\
     \hline
      Yang et al. \cite{yangetal} & 0.791 & 0.788 & 0.710\\
      \hline
      Xiao et al. \cite{xiaoetal} & 0.760 & 0.782 & 0.695 \\
      \hline
      CFSS \cite{cfss} & 0.784 & 0.783 & 0.713 \\
      \hline
      MTCNN \cite{MTCNN} & 0.748 & 0.760 & 0.726\\
      \hline
      MHM \cite{Jointalignment} & 0.847 & 0.838 & 0.769\\
      \hline
      MS-SFN (ours) & \textbf{0.901} & \textbf{0.884} & \textbf{0.842}\\
      \hline
    \end{tabular}
    \caption{Landmark localization performance of our method on videos in comparison to state-of-the-art face tracking methods. The values are reported in terms of Area under the Curve (AUC) for Cumulative Error Distribution of the 2D landmark error for 300VW test set.}
    \label{table:300vw_auc}
\end{table}

\begin{figure*}[h!]
\centering
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.1\textheight]{images/showcase/1130084326.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.1\textheight]{images/showcase/24795717.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.1\textheight]{images/showcase/5082623456.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.1\textheight]{images/showcase/4_Dancing_Dancing_4_357.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.1\textheight]{images/showcase/35_Basketball_basketballgame_ball_35_993.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.1\textheight]{images/showcase/39_Ice_Skating_Ice_Skating_39_696.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.1\textheight]{images/showcase/1130084326_3d.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.1\textheight]{images/showcase/24795717_3d.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.1\textheight]{images/showcase/5082623456_3d.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.1\textheight]{images/showcase/4_Dancing_Dancing_4_357_3d.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.1\textheight]{images/showcase/35_Basketball_basketballgame_ball_35_993_3d.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.16\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.1\textheight]{images/showcase/39_Ice_Skating_Ice_Skating_39_696_3d.jpg}
\end{subfigure}
\caption{Testing results of our joint detection and retargeting model. 
Column \textbf{1-3}: Sampled from AFW; Column \textbf{4-6}: Sampled from WIDER. We show both the predicted bounding boxes and the 3D meshes constructed from 3DMM parameters. }
\label{fig:result1}
\end{figure*}

\begin{table*}[t]
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{Model} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Eye\\ Close\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Eye\\ Wide\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Brow\\ Raise\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Brow\\ Anger\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Mouth\\ Open\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Jaw\\ L/R\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Lip\\ Roll\end{tabular}} & Smile & Kiss & \multicolumn{1}{c|}{Avg} \\ \hline
(1) Single scale SFN & 0.082   & 0.265   & 0.36   & 0.451   & 0.373   & 0.331   & 0.359   & 0.223 & 0.299 & 0.305 \\ \hline
(2) Multi-scale SFN & 0.016   & 0.257   & 0.216   & 0.381   & 0.334   & 0.131   & 0.204   & 0.245 & 0.277 & 0.229 \\ \hline
(3) MS-MFN + GT from (2) & 0.117   & 0.407   & 0.284   & 0.405   & 0.284   & 0.173   & 0.325   & 0.248 & 0.349 & 0.288 \\ \hline
\end{tabular}
\caption{Quantitative evaluation of expression accuracy (measured by the expression metric) on our expression test set. Lower error means the model performs better for extreme expressions when required.}
\label{table:exp}
\end{table*}



\begin{figure*}[h!]
\centering
\begin{subfigure}[t]{0.118\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.09\textheight]{images/showcase/2.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.118\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.09\textheight]{images/showcase/3.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.118\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.09\textheight]{images/showcase/5.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.118\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.09\textheight]{images/showcase/7.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.118\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.09\textheight]{images/showcase/21.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.118\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.09\textheight]{images/showcase/25.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.118\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.09\textheight]{images/showcase/27.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.118\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.09\textheight]{images/showcase/28.jpg}
\end{subfigure}

\begin{subfigure}[t]{0.118\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.09\textheight]{images/showcase/12.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.118\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.09\textheight]{images/showcase/13.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.118\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.09\textheight]{images/showcase/15.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.118\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.09\textheight]{images/showcase/17.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.118\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.09\textheight]{images/showcase/31.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.118\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.09\textheight]{images/showcase/35.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.118\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.09\textheight]{images/showcase/37.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.118\linewidth}
\includegraphics[width = 1.0\textwidth, height = 0.09\textheight]{images/showcase/38.jpg}
\end{subfigure}
\caption{Results by applying MS-SFN on our expression test set.}
\label{fig:result4}
\end{figure*}

\begin{figure*}[h!]
\centering
\includegraphics[width=1.0\linewidth]{images/retargetingresults.jpg}
\caption{Retargeting from face(s) to 3D character(s).}
\label{fig:retargeting}
\end{figure*}

\subsection{Importance of Joint Training}
Joint regression of both face bounding box locations and 3DMM parameters forces the network to learn exclusive facial features that characterize face shape, expression and pose in addition to differentiating face regions from the background. This helps in more precise face detection in-the-wild by leveraging both 2D information from bounding boxes and 3D information from 3DMM parameters. Table \ref{table:full} shows that average precision (AP) is improved by a large margin with joint training compared to when the same network is trained to only regress bounding box locations. The retargeting accuracy for MFN is also comparable to that of SFN and the slight decrease in NME is because of training MFN on multi-face images and testing on single face images. Nevertheless, we observe improved performance in terms of both NME and AP by using better ground truth generated by multi-scale model. Our detection accuracy (mAP: 98.8\%) outperforms Hyperface \cite{hyperface} (mAP: 97.9\%) and Faceness-Net \cite{facenessnet} (mAP: 97.2\%) on the entire AFW dataset when compared under the same settings. Results of our MFN on multi-face images are illustrated in Fig. \ref{fig:result1}.


\subsection{Evaluation of Expressions}
\iffalse
Our expression evaluation result in Table \ref{table:exp} emphasizes the improvement of multi-scale design on SFN. Since many applications can be created from expression (such as face rig avatar, emotion detection, etc.), it is important to maximize the expression coefficient when it should do. If the model itself can not predict large expression, the common approach is to apply post-processing by multiplying with heuristic number. This post-processing, however, can cause the retargeting result to shake. Most of the expressions are significantly better, however, MFN suffers from the small eye size (in comparison with the entire image). SFN, on the other hand, works on a cropped image, so eyes are zoomed in much further. Attention network for emphasizing small eyes region could be a future work for our MFN.
\fi

Our expression evaluation results in Table \ref{table:exp} emphasizes the improvement of multi-scale design on SFN. MS-MFN performs much better than SS-SFN for all expressions except the eye expressions. This is because eye patches are usually small compared to the entire image for MFN whereas they are zoomed in on cropped images for SFN. Attention network for emphasizing small eyes region could be a future work for our MFN. However, MS-MFN shows less accuracy compared to MS-SFN because it is being tested on single face images while being trained on multi-face images. For the multi-person test set images, we found similar visual results by applying MS-MFN on the whole image and by applying MS-SFN on each face individually cropped from the image. This is expected because MFN is trained with ground truth from SFN. The performance of MS-SFN on our expression test set is shown in Fig. \ref{fig:result4}. We also conducted live performance capture experiments to evaluate the efficiency our system in retargeting facial motion from one or more faces to one or more 3D characters. Fig. \ref{fig:retargeting} shows some screenshots recorded during the experiments.

\subsection{Computational Complexity}
Excluding the IO time, SFN can run at 15ms/frame on Google Pixel 2 (assuming single face and excluding face detector runtime). Face detection with our compressed detector model is 34ms, so separate face detection and retargeting requires 49ms for 1 face, 109ms for 5 faces and 184ms for 10 faces. On the other hand, our proposed MFN performs joint face detection and retargeting at 39ms on any number of faces. The model sizes for compressed face detector is 11.5MB and SFN is 2MB, so the combination is 13.5MB, while our MFN is only 13MB. Hence our joint network reduces both memory requirement and execution time.

%Model Comparison
\iffalse
\begin{table}[h]
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Method} & \multicolumn{2}{c|}{\textbf{NME (\%)}} & \multicolumn{2}{c|}{\textbf{MAE}}  \\ \hline
 {}      &        S1            &       S2         &    S1            &       S2            \\ \hline
Single-scale             &         2.21           &      -          &         0.218   & -    \\ \hline
Multi-scale      &         2.17           &       -         &           0.216   & -   \\ \hline
Proposed S1             &         1.91          &        -      &       0.215     & -     \\ \hline
S1 + S2 (sep)        &      1.91              &     1.62           &     0.215       &   0.209   \\ \hline
S1 + S2 (e2e)    &     1.47               &        1.82        &    0.212         &   0.222  \\ \hline
S1 + S2 (sep) + finetune         &        1.53           &      \textbf{1.25 }          &   0.207    &     \textbf{0.203}      \\ \hline
\end{tabular}
\caption {Normalized Mean Error of 68 landmarks and Mean Absolute Error of 46 expression parameters for LFW dataset (12639 images). S1 and S2 refers to Stage 1 and Stage 2 respectively.}
\end{table}

%Generalization to 29 Expression Basis
\begin{table}[h]
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Backbone} & \textbf{Size (MB)} & \textbf{GFLOP} & \textbf{Error} \\ \hline
State-of-the-art 1       &                    &                &                \\ \hline
State-of-the-art 2             &                    &                &                \\ \hline
State-of-the-art 3      &                    &                &                \\ \hline
Ours              &                    &                &                \\ \hline
\end{tabular}
\caption {Generalization to 29 Expression Basis Dataset}
\end{table}
\fi

\iffalse
\begin{figure}[t]
\centering
\begin{subfigure}[t]{1.0\linewidth}
\centering
\begin{subfigure}[t]{0.15\textwidth}
\centering
%\footnotesize input-1\\
\includegraphics[width = 1.0\textwidth, height = 0.055\textheight]{img1.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.15\textwidth}
\centering
%\footnotesize input-2\\
\includegraphics[width = 1.0\textwidth, height = 0.055\textheight]{img2.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.15\textwidth}
\centering
%\footnotesize input-3\\
\includegraphics[width = 1.0\textwidth, height = 0.055\textheight]{img3.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.15\textwidth}
\centering
%\footnotesize input-1\\
\includegraphics[width = 1.0\textwidth, height = 0.055\textheight]{img4.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.15\textwidth}
\centering
%\footnotesize input-2\\
\includegraphics[width = 1.0\textwidth, height = 0.055\textheight]{img5.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.15\textwidth}
\centering
%\footnotesize input-3\\
\includegraphics[width = 1.0\textwidth, height = 0.055\textheight]{img6.jpg}
\end{subfigure}
\caption{Input human images}
\end{subfigure}

\begin{subfigure}[t]{1.0\linewidth}
\centering
\begin{subfigure}[t]{0.15\textwidth}
\centering
%\footnotesize output-1\\
\includegraphics[width = 1.0\textwidth, height = 0.055\textheight]{mesh1.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.15\textwidth}
\centering
%\footnotesize output-2\\
\includegraphics[width = 1.0\textwidth, height = 0.055\textheight]{mesh2.jpg}
\end{subfigure}
%\caption{}
\begin{subfigure}[t]{0.15\textwidth}
\centering
%\footnotesize output-3\\
\includegraphics[width = 1.0\textwidth, height = 0.055\textheight]{mesh3.jpg}
\end{subfigure}
%\caption{}
\begin{subfigure}[t]{0.15\textwidth}
\centering
%\footnotesize output-1\\
\includegraphics[width = 1.0\textwidth, height = 0.055\textheight]{mesh4.jpg}
\end{subfigure}
\begin{subfigure}[t]{0.15\textwidth}
\centering
%\footnotesize output-2\\
\includegraphics[width = 1.0\textwidth, height = 0.055\textheight]{mesh5.jpg}
\end{subfigure}
%\caption{}
\begin{subfigure}[t]{0.15\textwidth}
\centering
%\footnotesize output-3\\
\includegraphics[width = 1.0\textwidth, height = 0.055\textheight]{mesh6.jpg}
\end{subfigure}
\caption{Output 3D meshes}
\end{subfigure}
\caption{
Facial retargeting results. This example shows (a) six different human images with different expressions and different head poses (b) retargeted 3D face meshes.}  
\label{mh2c}
\end{figure}
\fi

\iffalse
\subsubsection{Importance of multi-scale features}
Recent works on pose estimation have shown satisfactory performance using just the eye, nose and mouth corner landmarks, which indicates that pose estimation requires global features. Identity or shape of the face depends on the face contour landmarks along with the corners, hence they require region-based features. However, estimation of expression parameters requires a dense arrangement of landmarks and hence requires local features from the input image. This motivated us to combine features at different scales for different parameters. The low level layers of a CNN learn the local features, whereas the high level layers capture the global information.

\subsubsection{Importance of decoupling}
When we used only 2D landmark loss for optimization, we found that the combination of identity, expression and pose parameters learned by the model to fit the landmarks is different from the ground truth, although the output landmarks looked correct. This proves that due to sparsity of the 2D landmarks and the weak perspective projection approximation, the learned parameters may not be ideally distributed unless constrained individually.

\subsubsection{Importance of aligned refinement}
\begin{itemize}
\itemsep0em
\item In-plane rotation of the images before the refinement stage reduces the ambiguity in the data and helps the small network to quickly learn the details about the expression without worrying about the head pose.
\item Training the RefineNet with separate branches for the eye region and the mouth region helps in disentangling the relationship between the eye and mouth blendshapes apart from making it easier for the small network to concentrate on a smaller region.
\item Estimating only the update value of the expression parameters instead of predicting them from scratch helps in faster convergence.
\end{itemize}
We tried finetuning the expression branch in the CoarseNet by fixing all other branches after convergence, but we did not observe noticeable improvement.

\subsection{Comparison with state-of-the-art methods}

\subsubsection{Importance of having our new dataset(for expression)}

1.state of the art technique + old training set + old testing set\\
2. state of the art technique + old training set + our testing set\\
3. state of the art technique + our training set + our testing set\\
4. our technique + old training set + old testing set\\
5. our technique + our training set + our testing set\\

4VS1\& 2 - our technique is about the same for alignment purposes

5VS3 - our technique is designed to tailor the expression transfer


no worries about the complexity of model size, can we come up a compression technique


\subsection{train for tracking}

\subsubsection{Importance of our new DNN design(end2end comparison with state of the art)}

\subsubsection{2D Face Alignment Methods}

3DDFA and SDM\\
Evaluation metric: Normalized Mean Error, normalized by the face bounding box size.

Data-sets: AFLW and AFLW-20003D,
What to compare? : 68 and 21 facial landmark errors


\subsubsection{3D Face Reconstruction Methods}

Richardson (supervised) and Tewari (unsupervised).\\
Evaluation metric: Normalized Average Depth Error (NADE), normalized by the maximum depth of the neutral 3D mesh (generally a heatmap diagram) and Mean Absolute Error (MAE) of all the 3D vertices.

\subsection{Performance Analysis}

Our model is super light-weight, only occupying 1.8 MB of memory. The processing speed of our model is about 25 ms per image on a standard Android mobile device.
\fi

==> sec7_conclusion.tex <==
\section{Conclusion}
We propose a lightweight multitask learning network for joint face detection and facial motion retargeting on mobile devices in real time. The lack of 3DMM training data for multiple faces is tackled by generating weakly supervised ground truth from a network trained on images with single faces. We carefully design the network structure and regularization to enforce disentangled representation learning inspired by key observations. Extensive results have demonstrated the effectiveness of our design.

\textbf{Acknowledgements} We thank the anonymous reviewers for their constructive feedback, Muscle Wu, Xiang Yan, Zeyu Chen and Pai Zhang for helping, and Linda Shapiro, Alex Colburn and Barbara Mones for valuable discussions.
